Identification of 27 abnormalities from multi-lead ECG signals: An ensembled Se-ResNet framework with Sign Loss function

Cardiovascular disease is a major threat to health and one of the primary causes of death globally. The 12-lead ECG is a cheap and commonly accessible tool to identify cardiac abnormalities. Early and accurate diagnosis will allow early treatment and intervention to prevent severe complications of cardiovascular disease. In the PhysioNet/Computing in Cardiology Challenge 2020, our objective is to develop an algorithm that automatically identifies 27 ECG abnormalities from 12-lead ECG recordings.

==> declaration.tex <==
% this is only needed for a thesis
\newpage{}
  \thispagestyle{empty}
  \begin{center}
  \vspace*{1.5cm}
  {\LARGE Declaration }
  \end{center}
  \vspace{0.5cm}
  \begin{verse}
  \begin{center} 
I declare that this thesis is entirely my own work, and except where otherwise stated, describes
my own research.
\par

  \vspace{2.5cm}

B. S. Smoot,
\par
Smoot College
  \end{center}\end{verse}



==> dedication.tex <==
% this is only needed for a thesis
This thesis is dedicated to ... 
\par
This is optional and should only be included in a DPhil.
Do not include this section for PRS, MSc, MEng, Summer Reports etc.


